Optimal bounds for sign-representing the intersection of two halfspaces by polynomials

The threshold degree of a function f:{0,1}^n->{-1,+1} is the least degree of a real polynomial p with f(x)=sgn p(x). We prove that the intersection of two halfspaces on {0,1}^n has threshold degree Omega(n), which matches the trivial upper bound and completely answers a question due to Klivans (2002). The best previous lower bound was Omega(sqrt n). Our result shows that the intersection of two halfspaces on {0,1}^n only admits a trivial 2^{Theta(n)}-time learning algorithm based on sign-representation by polynomials, unlike the advances achieved in PAC learning DNF formulas and read-once Boolean formulas. The proof introduces a new technique of independent interest, based on Fourier analysis and matrix theory.

==> TODO <==
		-- In Equation (1.1), I suppose that the
		Beigel/Reingold/Spielman result is why you need the
		ratio to be exponential in n; maybe mention this?

>>>> KEEP AS IS


		-- It's a bit awkward in Lemma 3.2 and elsewhere to
		have "delta" occuring with two different meanings (as a
		small constant, and denoting a delta-function); even
		though there is no real ambiguity it would be better to
		use a different letter for the constant.

>>>> DONE


		-- Can you rephrase the definition of the function g
		(middle p. 6) in a different way?  The existential
		phrasing ("for some nonnegative integers ...) is
		perhaps not the most intuitive way.

>>>> DONE



		-- After the 2nd sentence of Sec 4, perhaps add brief
		mention that this is achieved by taking k to be a small
		constant multiple of n.

>>>> KEEP AS IS

	-- near bottom p. 7:  fix "It actuality,"  In the very
	last sentence of that page, perhaps cite the
	[Goldmann-Hastad-Razborov] or Hajnal et al paper as
	justification for why (4.3) rules out such a \mu.

>>>> DONE 

	-- Can you get an explicit construction? Is this
	question at all interesting?  Perhaps discuss this.

>>> KEEP AS IS


